Neutral Kaon Mixing Beyond the Standard Model with $n_f=2+1$ Chiral Fermions Part 1: Bare Matrix Elements and Physical Results

We compute the hadronic matrix elements of the four-quark operators relevant for $K^0-{\bar K^0}$ mixing beyond the Standard Model. Our results are from lattice QCD simulations with $n_f=2+1$ flavours of domain-wall fermion, which exhibit continuum-like chiral-flavour symmetry. The simulations are performed at two different values of the lattice spacing ($a\sim0.08$ and $a\sim 0.11 \, \fm $) and with lightest unitary pion mass $\sim 300\, \MeV$. For the first time, the full set of relevant four-quark operators is renormalised non-perturbatively through RI-SMOM schemes; a detailed description of the renormalisation procedure is presented in a companion paper. We argue that the intermediate renormalisation scheme is responsible for the discrepancies found by different collaborations. We also study different normalisations and determine the matrix elements of the relevant four-quark operators with a precision of $\sim 5\%$ or better.

==> Sections/s5_concl_bck.tex <==
\section*{Conclusions}\label{sec:concl}

We have computed the matrix elements necessary for beyond the Standard Model contributions to neutral Kaon mixing.
As previous studies have shown, the ratio of BSM contribution to SM is large. We have used a fermion discretisation
that has good chiral properties and extended our previous work with the addition of a second lattice spacing,
allowing us to extrapolate our results to the continuum. We notice that discretisation effects are significant and
although the $G_{ij}$ are chirally well behaved their continuum extrapolations can have a large slope in $a^2$.

%\commentnic{I add the table at $2$ GeV, also I show more s.f.}


\begin{table}[h]
\centering
\begin{tabular}{c|c c c c}
  \toprule
%  Intermediate Scheme & $R_2^{\rismom}(\mu)$ & $R_3^{\rismom}(\mu)$ & $R_4^{\rismom}(\mu)$ & $R_5^{\rismom}(\mu)$ \\
    Scheme & $R_2$ & $R_3$ & $R_4$ & $R_5$ \\
  \hline
  $\gmugmu$ & -19.11(53) & 5.76(22) & 40.1(21) & 11.13(85) \\
  $\qq$     & -20.31(55) & 6.12(24) & 42.7(21) & 10.68(84) \\
  \hline
 % Intermediate Scheme & $R_2^{\msbar}(\mu)$ & $R_3^{\msbar}(\mu)$ & $R_4^{\msbar}(\mu)$ & $R_5^{\msbar}(\mu)$ \\
  \hline
%$\gmugmu$ & -19.5(6) & 6.1(2) & 43.1(22) & 11.0(8) \\
%$\qq$ & -19.9(5) & 6.2(3) & 44.3(22) & 10.7(9) \\
$\msbar\leftarrow\gmugmu$ & -19.48(55) & 6.08(24) & 43.1(22) & 10.99(84) \\
$\msbar\leftarrow\qq$     & -19.91(54) & 6.22(26) & 44.3(22) & 10.68(85) \\
  \botrule
\end{tabular}
\caption{\raggedright{
    The ratios $R_i$ in the two intermediate $\rismom$ schemes and converted to $\msbar$.
    The renormalisation is performed at $\mu=3\;\text{GeV}$.
    Statistical and systematic errors have been added in quadrature.
   }}\label{conclusions:tab:rsmsbar}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{c|c c c c}
  \toprule
    Scheme & $R_2$ & $R_3$ & $R_4$ & $R_5$ \\
  \hline
  $\gmugmu$ & -15.77(42) & 4.88(14) & 30.7(13) & 8.27(44) \\
  $\qq$     & -17.19(46) & 5.30(16) & 33.4(14) & 7.79(42) \\
  \hline
%  Intermediate Scheme & $R_2^{\msbar}(\mu)$ & $R_3^{\msbar}(\mu)$ & $R_4^{\msbar}(\mu)$ & $R_5^{\msbar}(\mu)$ \\
  \hline
$\msbar\leftarrow\gmugmu$ & -16.14(43) & 5.20(15) & 33.5(14) & 8.15(44) \\
$\msbar\leftarrow\qq$     & -16.78(45) & 5.41(16) & 34.9(15) & 7.78(42) \\
  \botrule
\end{tabular}
\caption{\raggedright{
    Same as the previous table but the renormalisation is performed at $\mu=2\;\text{GeV}$.
    %Statistical and systematic errors have been added in quadrature, we have not attempted to estimate the perturbative truncation systematic but believe it to be small.
}}\label{conclusions:tab:rsmsbar2GeV}
\end{table}

We have renormalised our quantities non-perturbatively and have introduced two new SMOM schemes
which use non-exceptional kinematics rather than the previously used $\rimom$ (exceptional) scheme.
We argue that discrepancies between previous results are largely due to scheme dependence and in
particular the choice of intermediate momentum scheme. We strongly advocate the use of
the non-exceptional schemes defined in this work.
%as their matchings to $\msbar$ have smaller perturbative truncation systematics
%and they dramatically reduce chirally forbidden operator mixings under renormalisation.
We present what we consider to be the most important result of this work in table~\ref{conclusions:tab:rsmsbar},
these are the ratios renormalised at $3\;\text{GeV}$ in the $\msbar$ scheme from our two SMOM schemes.

We see that our systematics are dominated by the continuum extrapolation. We do not believe an increase in statistics
or simulation at physical pion and strange masses will be as beneficial as a third, finer lattice spacing.

%\commentnic{remove the discussion on PT, it is already in the results section}
% about PT, should put this somewhere else
%Not only this uncertainty can be important, but it is also
%the most difficult to estimate.
%Therefore we choose  $\mu=3$ for our central value: at this scale, the difference between the two schemes
%is significantly smaller than the other uncertainties.




==> Tables/table_schemes_bck.tex <==
\begin{table}[t]
\begin{tabular}{l | ccccc }
\toprule
& - & $R_2$ & $R_3$ & $R_4$ & $R_5$ \\
\cline{2-6}
$\gmugmu$ & - & -19.11(43)(31) & 5.76(14)(16) & 40.12(82)(188) & 11.13(21)(83) \\
$\qq$     & - & -20.31(46)(31) & 6.12(15)(19) & 42.74(88)(195) & 10.68(20)(82) \\
RI-MOM    & - & -15.77(33)(60) & 5.39(13)(9)  & 30.75(59)(217) &  7.24(11)(91) \\
\cline{2-6}
& $B_1$ & $B_2$ & $B_3$ & $B_4$ & $B_5$ \\
\cline{2-6}
$\gmugmu$ & 0.523(9)(7)  & 0.526(8)(18)  & 0.774(14)(65)  & 0.940(12)(11) & 0.786(9)(38) \\
$\qq$     & 0.541(9)(6)  & 0.523(8)(19)  & 0.770(14)(66)  & 0.937(12)(11) & 0.708(8)(38) \\
RI-MOM    & 0.517(9)(9)  & 0.571(8)(6)   & 0.950(17)(49)  & 0.947(10)(49) & 0.677(8)(81) \\
\cline{2-6}
& - & $G_{21}$ & $G_{23}$ & $G_{24}$ & $G_{45}$ \\
\cline{2-6}
$\gmugmu$ & - & 1.005(13)(46) & 0.664(2)(21) & 0.502(13)(10) & 1.175(6)(56)\\
$\qq$     & - & 0.967(13)(42) & 0.664(2)(21) & 0.498(13)(10) & 1.296(8)(72)\\
RI-MOM    & - & 1.105(13)(6) & 0.590(2)(27) & 0.549(11)(34) & 1.266(18)(181)\\
\botrule
& - & $R_2$ & $R_3$ & $R_4$ & $R_5$ \\
\cline{2-6}
$\msbar \leftarrow \gmugmu$ & - & -19.48(44)(53)  & 6.08(15)(23)  & 43.11(89)(230)  & 10.99(20)(88) \\
$\msbar \leftarrow \qq$     & - & -19.91(45)(53)  & 6.22(16)(25)  & 44.25(91)(232)  & 10.68(20)(88) \\
$\msbar \leftarrow$ RI-MOM  & - & -16.44(36)(44)  & 5.31(13)(15)  & 34.56(68)(204)  &  8.50(14)(89) \\
\cline{2-6}
& $B_1$ & $B_2$ & $B_3$ & $B_4$ & $B_5$ \\
\cline{2-6}
$\msbar \leftarrow \gmugmu$ & 0.525(9)(13)  & 0.488(7)(17)  & 0.743(14)(65)  & 0.920(12)(16)  & 0.707(8)(44) \\
$\msbar \leftarrow \qq$     & 0.536(9)(13)  & 0.492(7)(18)  & 0.751(14)(66)  & 0.932(12)(17)  & 0.680(8)(45) \\
$\msbar \leftarrow$ RI-MOM  & 0.526(9)(9)   & 0.417(6)(2)   & 0.655(12)(44)  & 0.745(9)(28)   & 0.555(6)(53) \\
\cline{2-6}
& - & $G_{21}$ & $G_{23}$ & $G_{24}$ & $G_{45}$ \\
\cline{2-6}
$\msbar \leftarrow \gmugmu$ & - & 0.930(12)(59) & 0.642(2)(34) & 0.456(12)(20) & 1.278(7)(64)   \\
$\msbar \leftarrow \qq$     & - & 0.920(12)(57) & 0.641(2)(34) & 0.467(12)(21) & 1.342(8)(78)   \\
$\msbar \leftarrow$  RI-MOM & - & 0.793(10)(16) & 0.621(2)(28) & 0.316(7)(12)  & 1.267(12)(125) \\
\botrule
\end{tabular}
\caption{\raggedright{Final results for $R_i$, $B_i$ and $G_{ij}$ renormalised at $\mu=3\,\text{GeV}$.
    The first error is statistical and the second is the total systematic error.
    The RI-MOM results are  presented here only for illustration and comparison purposes.
    Our best results are the ones obtained through the SMOM-$\gmugmu$ and $\qq$ schemes.
    For the $\msbar \leftarrow \gmugmu$ and $\msbar \leftarrow \qq$ results,
    the systematic errors include the estimate of the perturbative errors.
    This error is not included for the $\msbar \leftarrow \rm RI-MOM$ case.
  }\label{results:tab:final_results}}
\end{table}

